Music Sequence Prediction with Mixture Hidden Markov Models

Recommendation systems that automatically generate personalized music playlists for users have attracted tremendous attention in recent years. Nowadays, most music recommendation systems rely on item-based or user-based collaborative filtering or content-based approaches. In this paper, we propose a novel mixture hidden Markov model (HMM) for music play sequence prediction. We compare the mixture model with state-of-the-art methods and evaluate the predictions quantitatively and qualitatively on a large-scale real-world dataset in a Kaggle competition. Results show that our model significantly outperforms traditional methods as well as other competitors. We conclude by envisioning a next-generation music recommendation system that integrates our model with recent advances in deep learning, computer vision, and speech techniques, and has promising potential in both academia and industry.

==> figure_hmm_demo.tex <==
\begin{figure*}[!ht]
\centering
\includegraphics[width=3in]{hmm_demo.png}
\caption[HMM]{Demonstration of hidden Markov models\footnote{\url{https://stathwang.github.io/part-of-speech-tagging-with-trigram-hidden-markov-models-and-the-viterbi-algorithm.html}}}
\label{fig:hmm-demo}
\end{figure*}


==> figure_ranking.tex <==
% \begin{figure*}[!ht]
% \centering
% \subfloat[competition panel]{\includegraphics[width=2.25in]{panel.png}
% \label{fig:panel}}
% \hfil
% \subfloat[final rankings and scores]{\includegraphics[width=2.25in]{ranking.png}
% \label{fig:ranking}}
% \caption{Kaggle Competition: Music Sequence Prediction}
% \label{fig:ranking}
% \end{figure*}
\begin{figure*}[!ht]
% \centering
\includegraphics[width=2.25in]{ranking.png}
\label{fig:ranking}
\caption{Kaggle Competition Final Leaderboard}
\end{figure*}


==> table_setting.tex <==
\begin{table}[!t]
\caption{Experimental settings}
\label{tab:setting}
\centering
\begin{tabular}{ | l | r | }
% \hline
% Model & MAP@K \\
\hline
$\mathbb{N}$ & $972$ \\
$\mathbb{K}$ & $10$ \\
% $y_i$ & $30^{th}$ artist \\
\hline
\end{tabular}
\end{table}

